Expert Knowledge-Guided Length-Variant Hierarchical Label Generation for Proposal Classification

To advance the development of science and technology, research proposals are submitted to open-court competitive programs developed by government agencies (e.g., NSF). Proposal classification is one of the most important tasks to achieve effective and fair review assignments. Proposal classification aims to classify a proposal into a length-variant sequence of labels. In this paper, we formulate the proposal classification problem into a hierarchical multi-label classification task. Although there are certain prior studies, proposal classification exhibit unique features: 1) the classification result of a proposal is in a hierarchical discipline structure with different levels of granularity; 2) proposals contain multiple types of documents; 3) domain experts can empirically provide partial labels that can be leveraged to improve task performances. In this paper, we focus on developing a new deep proposal classification framework to jointly model the three features. In particular, to sequentially generate labels, we leverage previously-generated labels to predict the label of next level; to integrate partial labels from experts, we use the embedding of these empirical partial labels to initialize the state of neural networks. Our model can automatically identify the best length of label sequence to stop next label prediction. Finally, we present extensive results to demonstrate that our method can jointly model partial labels, textual information, and semantic dependencies in label sequences, and, thus, achieve advanced performances.

==> appedix.tex <==
\section{Appendix}
\label{appendix}

\subsection{Transformer Details}
A layer of transformer encoder (i.e, a transformer block) consists of a \textit{Multi-Head Self-Attention Mechanism}, a \textit{Residual Connections and Layer Normalization Layer}, a \textit{Feed Forward Layer}, and a \textit{Residual Connections and  Normalization Layer}, which can be written as:

\begin{equation}
    H = LayerNorm(X^{(l)}+MultiHead(X^{(l)}))
\end{equation}

\begin{equation}
    X^{(l+1)} =  LayerNorm(H+MLP(H))
\end{equation}

where $X^{(l)} = \{x_1^{(l)}, x_2^{(l)}, ..., x_s^{(l)}\}$ is the input sequence of $l$-th layer of transformer, $s$ is the length of input sequence, $ x_i^{(l)}\in \mathbb{R}^d$ and $d$ in the dimension. LayerNorm is layer normalization, MLP denotes a two-layer feed-forward network with ReLU activation
function, and MultiHead denotes the multi-head attention mechanism, which is
calculated as follows:

\begin{equation}
MultiHead(X^{(k)}) = Concat (head_1, . . . , head_h)W^O
\end{equation}

\begin{equation}
head_i = Attention(Q,K,V)
\end{equation}

\begin{equation}
Attention (Q,K,V) = softmax(\frac{QK^T}{\sqrt{d}})V
\end{equation}

\begin{equation}
\begin{aligned}
where  \  & Q = X^{(l)} W_i^Q,  \\
& K = X^{(l)} W_i^K,  \\
& V = X^{(l)} W_i^V  \\
\end{aligned}
\end{equation}

where $W_i^Q, W_i^K, W_i^V\in \mathbb{R}^{d\times d}$ are weight metrics, The $h$ outputs from the attention calculations are concatenated and
transformed using a output weight matrix $W^O\in \mathbb{R}^{dh\times d}$. The main hyper-parameters of a transformer are the number of layers (i.e., transformer blocks), the number of self-attention heads, and the maximum length of inputs. 

Given the input sequence embeddings $X^{(0)} = \{x_1^{(0)}, x_2^{(0)}, ..., x_l^{(0)}\}$, after the propagation on $L$-layers transformer, we can obtain the final output embeddings of this sequence $X^{(L)} = \{x_1^{(L)}, x_2^{(L)}, ..., x_l^{(L)}\}$, where each embedding has contained the context information in this sequence.

